RFRL Gym: A Reinforcement Learning Testbed for Cognitive Radio Applications

Radio Frequency Reinforcement Learning (RFRL) is anticipated to be a widely applicable technology in the next generation of wireless communication systems, particularly 6G and next-gen military communications. Given this, our research is focused on developing a tool to promote the development of RFRL techniques that leverage spectrum sensing. In particular, the tool was designed to address two cognitive radio applications, specifically dynamic spectrum access and jamming. In order to train and test reinforcement learning (RL) algorithms for these applications, a simulation environment is necessary to simulate the conditions that an agent will encounter within the Radio Frequency (RF) spectrum. In this paper, such an environment has been developed, herein referred to as the RFRL Gym. Through the RFRL Gym, users can design their own scenarios to model what an RL agent may encounter within the RF spectrum as well as experiment with different spectrum sensing techniques. Additionally, the RFRL Gym is a subclass of OpenAI gym, enabling the use of third-party ML/RL Libraries. We plan to open-source this codebase to enable other researchers to utilize the RFRL Gym to test their own scenarios and RL algorithms, ultimately leading to the advancement of RL research in the wireless communications domain. This paper describes in further detail the components of the Gym, results from example scenarios, and plans for future additions. Index Terms-machine learning, reinforcement learning, wireless communications, dynamic spectrum access, OpenAI gym

==> sections/GUI.tex <==
% this is not being included in the final product at the moment but keeping unless it needs to be referenced
\section{Graphical User Interface Overview}
%A graphical user interface (GUI) is a type of user interface that allows users to interact with the RFRL Gym through graphical elements. This was developed with the intention of making the RFRL Gym accessible for people of all backgrounds, who are interested in radio frequency and reinforcement learning. The abstraction of the code and the integration of GUI focuses on reducing the margins for errors and assisting users in concentrating on their research and data analysis by simplifying the process. 
%made the above a comment for now, since this has already been stated in the background section... idk if it's necessary. 

       Currently, there are two interfaces available in our package that improve the accessibility of the RFRL Gym: the Scenario Selection Graphical User Interface (GUI) and the Gym Rendering Modes. Below the Scenario Selection GUI will be discussed in more detail. 

       A Scenario Selection GUI has been designed with the intent of simplifying the creation of a scenario file. The GUI enables the modification and creation of scenario files without interfacing with a JSON file directly. This simplifies the process of creating scenario files because syntax does not need to be memorized and non-software-oriented users can produce scenarios.  Fig. 4 shows the layout of the GUI.There are many planned enhancements for the GUI that will be covered in the future work section. 
    
       
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/scenarioGUI.png}
    \caption{Scenario generator for user interface}
    \label{fig:my_label}
\end{figure}


       When the user navigates to the Environment sub-section, they can personalize the number of channels, the maximum time step, the observation mode, and the reward types. In the Entity sub-section, the user can add a variety of entity types and specify their behavior patterns. additionally the user has the capacity to tailor the non-player entities to their expectations.There will also be a visualization of how the entities will behave. In the Render sub-section, the user has the ability to modify the rendering mode and adjust the speed of the render visualization. Lastly, there is a Scenario Overview sub-section that will allow the user to determine if there are any other changes they want to make to their custom scenario before exporting it to an official scenario file. 

       
       
